Large Language Model for Discrete Optimization Problems: Evaluation and Step-by-step Reasoning

This work investigated the capabilities of different models, including the Llama-3 series of models and CHATGPT, with different forms of expression in solving discrete optimization problems by testing natural language datasets. In contrast to formal datasets with a limited scope of parameters, our dataset included a variety of problem types in discrete optimization problems and featured a wide range of parameter magnitudes, including instances with large parameter sets, integrated with augmented data. It aimed to (1) provide an overview of LLMs' ability in large-scale problems, (2) offer suggestions to those who want to solve discrete optimization problems automatically, and (3) regard the performance as a benchmark for future research. These datasets included original, expanded and augmented datasets. Among these three datasets, the original and augmented ones aimed for evaluation while the expanded one may help finetune a new model. In the experiment, comparisons were made between strong and week models, CoT methods and No-CoT methods on various datasets. The result showed that stronger model performed better reasonably. Contrary to general agreement, it also showed that CoT technique was not always effective regarding the capability of models and disordered datasets improved performance of models on easy to-understand problems, even though they were sometimes with high variance, a manifestation of instability. Therefore, for those who seek to enhance the automatic resolution of discrete optimization problems, it is recommended to consult the results, including the line charts presented in the Appendix, as well as the conclusions drawn in this study for relevant suggestions.

==> Figures.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{statistic.jpg}
\caption{Statistics on the Number of Variables}
\label{fig1}
\end{figure}

\begin{figure}[h] % [h]表示图片尽量放在此处
    \centering % 使图片居中
    \includegraphics[width=0.65\textwidth]{graph2.jpg} % 插入图片，文件名不需要后缀
    \caption{AR/PR Ratio Across Specified Parameter Range with DeepSeek-Implicit on Different Problems} % 图片标题
    \label{model2} % 图片标签，用于引用
\end{figure}

\begin{figure}[h] % [h]表示图片尽量放在此处
    \centering % 使图片居中
    \includegraphics[width=\textwidth]{graph1.jpg} % 插入图片，文件名不需要后缀
    \caption{AR/PR Ratio Across Specified Parameter Range with LLAMA3-Implicit on Different Problems} % 图片标题
    \label{model1} % 图片标签，用于引用
\end{figure}

\begin{figure}[h] % [h]表示图片尽量放在此处
    \centering % 使图片居中
    \includegraphics[width=0.74\textwidth]{graph3.jpg} % 插入图片，文件名不需要后缀
    \caption{AR/PR Ratio Across Specified Parameter Range with GPT-4o-mini-CoT-Implicit on Different Problems} % 图片标题
    \label{model3} % 图片标签，用于引用
\end{figure}

\begin{figure}[h] % [h]表示图片尽量放在此处
    \centering % 使图片居中
    \includegraphics[width=0.74\textwidth]{graph4.jpg} % 插入图片，文件名不需要后缀
    \caption{AR/PR Ratio Across Specified Parameter Range with LLAMA3-CoT-Implicit-Disorder on Different Problems} % 图片标题
    \label{model4} % 图片标签，用于引用
\end{figure}




==> tables.tex <==
\usepackage{tabularx}
\usepackage{adjustbox}
\usepackage{longtable}
\usepackage{changepage}

\begin{table}[htbp]
  \caption{Basic Information of Each Type of Problems (Part 1)}
  \label{table1}
  \centering
  \scriptsize            % 如需更小字号可改为 \tiny
  \renewcommand{\arraystretch}{1.2}  % 调整行高
  \setlength{\tabcolsep}{4pt}        % 缩小列间距
  \begin{adjustbox}{} 
    \begin{tabularx}{\textwidth}{@{}lXr@{\hspace{6mm}}lXr@{}}
      \toprule
      \multicolumn{3}{c@{\hspace{6mm}}}{\textbf{Left Section}} & \multicolumn{3}{c}{\textbf{Right Section}} \\
      \cmidrule(lr){1-3} \cmidrule(l){4-6}
      \textbf{Problems} & \textbf{Mathematical Model} & \textbf{Number of Instances}
        & \textbf{Problems} & \textbf{Mathematical Model} & \textbf{Number of Instances} \\
      \midrule

      Assignment &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{i=1}^n\sum_{j=1}^n c_{ij}\,x_{ij},\\
\text{s.t. } 
& \sum_{i=1}^n x_{ij} = 1,\quad \forall\,j=1,\dots,n,\\
& \sum_{j=1}^n x_{ij} = 1,\quad \forall\,i=1,\dots,n,
\end{aligned}$ & 12
      &
      Steiner$^*$ &
      $\displaystyle
      \begin{aligned}[t]
&\min_{\textbf p\in\mathbb R^2}Z 
= \sum_{i=1}^n \bigl\|\textbf p - (x_i, y_i)\bigr\|_2 \\ 
&= \sum_{i=1}^n \sqrt{(p_x - x_i)^2 + (p_y - y_i)^2},
\end{aligned}$ & 196 \\
      \addlinespace[3pt]

      1D-Binpacking &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= m,\\
\text{s.t. } 
& \sum_{j=1}^m x_{ij} = 1,\quad \forall\,i=1,\dots,n,\\
& \sum_{i=1}^n w_i\,x_{ij} \le C,\quad \forall\,j=1,\dots,m,
\end{aligned}$ & 160
      &
      2D-cutting &
      $\displaystyle
      \begin{aligned}[t]
\max\;Z &= \sum_{j=1}^n p_j\,x_j,\\
\text{s.t. } 
& \sum_{j=1}^n a_j\,x_j \le A,\\
& \sum_{j=1}^n b_j\,x_j \le B,
\end{aligned}$ & 3 \\
      \addlinespace[3pt]

      Crew-scheduling &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{i=1}^n\sum_{j=1}^m c_{ij}\,x_{ij},\\
\text{s.t. } 
& \sum_{j=1}^m x_{ij} = 1,\quad \forall\,i=1,\dots,n,\\
& \sum_{i=1}^n t_i\,x_{ij} \le T_j,\quad \forall\,j=1,\dots,m,
\end{aligned}$ & 10
      &
      UBQP &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{i=1}^n\sum_{j=1}^n Q_{ij}\,x_i\,x_j,\\
\text{s.t. } 
& x_i \in \{0,1\},\quad i=1,\dots,n,
\end{aligned}$ & 45 \\
      \bottomrule
    \end{tabularx}
  \end{adjustbox}
\end{table}

\begin{table}[htbp]
  \caption{Basic Information of Each Type of Problems (Part 2)}
  \label{table11}
  \centering
  \scriptsize            % 如需更小字号可改为 \tiny
  \renewcommand{\arraystretch}{1.2}  % 调整行高
  \setlength{\tabcolsep}{4pt}        % 缩小列间距
  \begin{adjustbox}{} 
    \begin{tabularx}{\textwidth}{@{}lXr@{\hspace{6mm}}lXr@{}}
      \toprule
      \multicolumn{3}{c@{\hspace{6mm}}}{\textbf{Left Section}} & \multicolumn{3}{c}{\textbf{Right Section}} \\
      \cmidrule(lr){1-3} \cmidrule(l){4-6}
      \textbf{Problems} & \textbf{Mathematical Model} & \textbf{Number of Instances}
        & \textbf{Problems} & \textbf{Mathematical Model} & \textbf{Number of Instances} \\
      \midrule
        CVRP &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{i=0}^n\sum_{j=0}^n c_{ij}\,x_{ij},\\
\text{s.t. } 
& \sum_{j=1}^n x_{0j} = k,\\
& \sum_{j=0}^n x_{ij} = 1,\quad \forall\,i=1,\dots,n,\\
& \sum_{i=1}^n q_i\,x_{ij} \le Q,\quad \forall\,j=1,\dots,k,
\end{aligned}$ & 202
      &
      PVRP &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{i=0}^n\sum_{j=1}^n\sum_{k=1}^K c_{ij}\,x_{ijk},\\
\text{s.t. } 
& \sum_{k=1}^K y_{jk} = 1,\quad \forall\,j=1,\dots,n,\\
& \sum_{j=0}^n x_{0jk} = 1,\quad \forall\,k=1,\dots,K,\\
& \sum_{i=1}^n q_i\,x_{ijk} \le Q_k,\quad \forall\,k=1,\dots,K,
\end{aligned}$ & 42 \\
      \addlinespace[3pt]

      MDVRP &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{i=0}^n\sum_{j=1}^n\sum_{k=1}^K c_{ij}\,x_{ijk},\\
\text{s.t. } 
& \sum_{k=1}^K y_{jk} = 1,\quad \forall\,j=1,\dots,n,\\
& \sum_{j=0}^n x_{0jk} = 1,\quad \forall\,k=1,\dots,K,\\
& \sum_{i=1}^n q_i\,x_{ijk} \le Q_k,\quad \forall\,k=1,\dots,K,
\end{aligned}$ & 33
      &
      Aircraft Landing &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{i=1}^n d_i\,L_i,\\
\text{s.t. } 
& L_i \ge L_{i-1} + \sum_{j=1}^n T_{ij}\,x_{ij},\quad \forall\,i=2,\dots,n,\\
& \sum_{j=1}^n x_{ij} = 1,\quad \forall\,i=1,\dots,n,
\end{aligned}$ & 13 \\
      \addlinespace[3pt]

      Generalised Assignment &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{i=1}^n\sum_{j=1}^m c_{ij}\,x_{ij},\\
\text{s.t. } 
& \sum_{j=1}^m x_{ij} = 1,\quad \forall\,i=1,\dots,n,\\
& \sum_{i=1}^n w_{ij}\,x_{ij} \le W_j,\quad \forall\,j=1,\dots,m,
\end{aligned}$ & 60
      &
      Multi-Knapsack &
      $\displaystyle
      \begin{aligned}[t]
\max\;Z &= \sum_{i=1}^m\sum_{j=1}^n v_j\,x_{ij},\\
\text{s.t. } 
& \sum_{j=1}^n w_{ij}\,x_{ij} \le W_i,\quad \forall\,i=1,\dots,m,\\
& \sum_{i=1}^m x_{ij} \le 1,\quad \forall\,j=1,\dots,n,
\end{aligned}$ & 277 \\
      \addlinespace[3pt]

      Warehouse Location &
      $\displaystyle
      \begin{aligned}[t]
\min\;Z &= \sum_{j=1}^m f_j\,y_j \;+\; \\ & \sum_{i=1}^n\sum_{j=1}^m c_{ij}\,x_{ij},\\
\text{s.t. } 
& \sum_{j=1}^m x_{ij} = 1,\quad \forall\,i=1,\dots,n,\\
& \sum_{i=1}^n d_i\,x_{ij} \le Q_j\,y_j,\quad \forall\,j=1,\dots,m,
\end{aligned}$ & 34
      & & & \\
      \bottomrule
    \end{tabularx}
  \end{adjustbox}
\end{table}

\begin{table}[H]
\caption{Statistics on Various Datasets}%标题
\label{table2}
\centering%把表居中
\begin{tabular}{cccc}%四个c代表该表一共四列，内容全部居中
\toprule%第一道横线
PROBLEMS&MANUAL&EXPANDED&AUGMENTED\\
\midrule%第二道横线 
Assignment&60&48&108 \\
1D-Binpacking&960&640&1600 \\
Crew-scheduling&150&100&250 \\
Steiner&980&980&1960 \\
UBQP&135&90&225 \\
CVRP&606&404&1010 \\
MDVRP&132&88&220 \\
PVRP&126&84&210 \\
Aircraft Landing&26&26&52 \\
Generalised assignment&180&120&300 \\
Multi-dimensional knapsack&1108&841&1949 \\
Capacitated Warehouse Location&102&68&170 \\
2D-cutting Packing-constrained Guillotine&18&12&30 \\
\bottomrule%第三道横线
\end{tabular}
\end{table}

\begin{table}[h]
    \centering
    \caption{Error Types and Descriptions}
    \begin{tabular}{lp{10cm}} % 设置描述列宽度为10cm
        \toprule
        \textbf{Error Types} & \textbf{Description} \\
        \midrule
        IndexError & Raised when trying to access an index that is out of range for a list or a sequence. \\
        FileNotFoundError & Raised when a file or directory is requested but cannot be found. \\
        OverflowError & Raised when a calculation exceeds the limits of the data type, typically in numeric operations. \\
        NameError & Raised when a local or global name is not found, meaning the variable or function is not defined. \\
        ValueError & Raised when a function receives an argument of the right type but an inappropriate value, such as converting a non-numeric string to an integer. \\
        AttributeError & Raised when an invalid attribute reference is made, meaning the attribute does not exist on the object. \\
        KeyError & Raised when attempting to access a dictionary with a key that does not exist. \\
        SyntaxError & Raised when the Python interpreter encounters invalid syntax in the code, preventing execution. \\
        TypeError & Raised when an operation or function is applied to an object of inappropriate type, such as adding a string to an integer. \\
        ImportError & Raised when a module or package cannot be imported, often due to it not being found or having issues within it. \\
        PulpError & Raised in the context of optimization problems, indicating issues such as infeasibility or unbounded solutions. \\
        SolutionError & Raised when the solution of a problem is invalid, often related to disobeying constraints. \\
        ResultError & Raised when a function does not yield an expected form of result, often due to output error by LLMs. \\
        \bottomrule
    \end{tabular}
    \label{DESCRIPTION}
\end{table}

\begin{table}[!htbp]
    \centering
    \caption{A case study of 1D-Binpacking problem}
    \label{EXAMPLE}
    \begin{threeparttable}
        \begin{tabular}{p{0.4\textwidth} p{0.4\textwidth} @{}c@{}}
            \toprule
            \textbf{\textcircled{1}Implicit} & \textbf{\textcircled{1}Explicit} & 
            \multirow{4}{*}{\shortstack{\textcircled{1} \\ \rule{0.4pt}{15pt} \\ \rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\ \rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\$\downarrow$}} \\ % 合并4行
            \cmidrule(lr){1-2}
            \raggedright
            There are 120 items S and several boxes B with a capacity of 150. The volumes of the 120 items are \textbf{[BLANK]}, and it is given that $s_i \leq 150$ ($1\leq i \leq 120$). The packing problem seeks to pack all items into the boxes in such a way that the number of boxes used is minimized. The following table shows the volumes of the items: \textbf{[BLANK]}  
            & There are 120 items S and several boxes B with a capacity of 150. The volumes of the 120 items are $s_1, s_2, \ldots, s_{120}$, and it is given that $s_i \leq 150$ ($1 \leq i \leq 120$). The packing problem seeks to pack all items into the boxes in such a way that the number of boxes used is minimized. The following table shows the volumes of the items:
            $x_1$,$x_2$,{\ldots}, $x_{119}$,$x_{120}$&\\
            \cmidrule(lr){1-2}
            \multicolumn{2}{c}{\textbf{\textcircled{1}Implicit-Disorder}} &  \\
            \cmidrule(lr){1-2}
            \multicolumn{2}{p{0.8\textwidth}}{%
                \raggedright
                The packing problem seeks to pack all items into the boxes in such a way that the number of boxes used is minimized The following table shows the volumes of the items: $x_1$ $x_2$ {\ldots} $x_{119}$ $x_{120} s_{120}$, and it is given that $s_i \leq 150$ ($1\leq i\leq120$) 1.There are 120 items S and several boxes B with a capacity of 150. The volumes of the 120 items are $s_{1}, s_{2},$
            }\\
            \cmidrule(lr){1-2}
            \multicolumn{2}{c}{\textbf{\textcircled{2}CoT Prompting(Optional)}} & \multirow{4}{*}{\shortstack{\textcircled{2} \\ \rule{0.4pt}{15pt} \\ \rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\ \rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\\rule{0.4pt}{15pt} \\$\downarrow$}} \\ % 合并4行
            \cmidrule(lr){1-2}
            \multicolumn{2}{p{0.8\textwidth}}{%
  \raggedright
  Dealing with 1D bin‑packing problems involves several key steps. Here’s a concise outline: \\[0.5ex]
  1. Define the Problem: Clearly state the items to be packed (sizes and quantities) and the capacity of the bins. \\ 
  2. Choose a Strategy: Select a bin‑packing algorithm or heuristic (First‑Fit, Best‑Fit, FFD, BFD). \\  
  3. Sort the Items: If using a decreasing strategy, sort the items in descending order. \\ 
  4. Initialize Bins: Create an empty list or array to represent the bins. \\ 
  5. Pack the Items: Iterate through the sorted list and place each item into the first suitable bin. \\ 
  6. Handle Overflows: If an item cannot fit, create a new bin. \\ 
  7. Track Usage: Record how many bins are used and their contents. \\ 
  8. Evaluate the Solution: Assess packing efficiency (number of bins used, waste). \\ 
  9. Optimize (if needed): Explore further optimization techniques. \\ 
  10. Implement and Test: Run with various inputs to ensure correctness and efficiency.
}\\
            \cmidrule(lr){1-2}

            \multicolumn{2}{c}{\textbf{\textcircled{3}Common Prompting}} & \textcircled{3} \\ % 合并4行 \\
            \cmidrule(lr){1-2}
            \multicolumn{2}{p{0.8\textwidth}}{%
                \raggedright
                Output the python program that stores the optimum value into result and then into file: output.txt(only store optimum value without any redundant expression).
            } & \\
            \bottomrule
        \end{tabular}
    \end{threeparttable}
\end{table}

\begin{table}[ht]
\centering
\caption{PR Task Performance Comparison}
\label{PR}
\resizebox{\textwidth}{!}{% 
\begin{tabular}{llcccccccc}
\toprule
\multirow{2}{*}{Task} & \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{GPT-4o-mini} & \multicolumn{2}{c}{LLAMA3-8B} & \multicolumn{2}{c}{ORLM} & \multicolumn{2}{c}{DeepSeek-R1}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
 & & PoT & PoT+CoT & PoT & PoT+CoT &PoT & PoT+CoT &PoT & PoT+CoT \\
\midrule
\multirow{3}{*}{Assignment} 
& Explicit-origin & \textbackslash{}  & $76.67$ & \textbackslash{}   &  \textbackslash{} &  \textbackslash{} &  \textbackslash{} &  \textbackslash{} &  \textbackslash{}\\
& Implicit-origin & $80.88$  & $91.67$ & $9.09$  & $43.33$ &$0.00$&$8.33$ &\textbf{\textbf{98.33}}&$85.00$\\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{92.59}} & $13.89$  & $39.81$ & $0.93$  & $9.26$ & \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{1D-Binpacking}
& Explicit-origin & \textbackslash{}  & $83.37$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $64.06$  & $75.73$ & $55.21$  & $12.50$ & $3.54$ & $8.12$ & $80.47$ & \textbf{\textbf{82.55}}  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{83.19}} & $7.35$  & $9.96$ & $3.25$  & $3.98$ & \textbackslash{}  & \textbackslash{} \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Crew-scheduling}
& Explicit-origin & \textbackslash{}  & $76.00$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $52.00$  & $52.67$ & $4.67$  & $3.33$ & $0.00$ & $2.00$ & \textbf{\textbf{79.33}} & $67.59$  \\
& Implicit-disorder & \textbackslash{}  & $44.31$ & $3.60$  & $1.60$& \textbf{\textbf{72.31}}  & $0.80$ & \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Steiner}
& Explicit-origin & \textbackslash{}  & $84.48$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $87.86$  & $93.67$ & $20.73$  & $14.29$ & $1.12$ & $0.10$ & $76.30$ & \textbf{\textbf{97.10}}  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{23.54}} & $3.06$  & $13.68$ & $0.92$  & $1.86$ & \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{UBQP}
& Explicit-origin & \textbackslash{}  & 60.74 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $17.78$  & $62.69$ & $16.30$  & $8.89$ & $1.48$ & $2.96$ & $64.44$ & \textbf{\textbf{93.33}}  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{30.46}} & $14.67$  & $4.00$ & $0.89$  & $5.78$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{CVRP}
& Explicit-origin & \textbackslash{}  & $64.00$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $36.15$  & $47.06$ & $2.12$  & $0.49$ & $0.16$ & $0.49$ & $71.16$ & \textbf{\textbf{83.87}}  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{49.31} } & $3.04$  & $1.10$ & $0.59$  & $0.49$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{MDVRP}
& Explicit-origin & \textbackslash{}  & $53.79$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $75.76$  & $77.27$ & $0.76$  & $5.30$ & $0.00$ & $0.00$ & \textbf{\textbf{93.18}} & $46.21$ \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{75.76}} & $6.57$  & $2.02$& $0.51$  & $1.52$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{PVRP}
& Explicit-origin & \textbackslash{}  & $71.43$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $72.22$  & $67.46$ & $2.38$  & $2.38$&$0.79$&$0.00$&\textbf{\textbf{79.37}}&$71.31$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{73.81}} & $2.38$  & $2.38$& $0.00$  & $0.95$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Aircraft Landing}
& Explicit-origin & \textbackslash{}  & $56.82$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & \textbf{\textbf{77.27}}  & $68.18$ & $11.36$  & $9.09$&$0.00$&$0.00$&$68.18$&$0.00$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{67.05}} & $18.18$  & $7.95$& $0.00$  & $1.14$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Generalised Assignment}
& Explicit-origin & \textbackslash{}  & $70.56$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & \textbf{\textbf{76.11}}  & $58.89$ & $6.67$  &$6.67$&$1.67$&$1.67$&$24.00$&$53.85$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{76.00}} & $8.00$  & $5.00$& $2.33$  & $1.33$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Multi-dimensional Knapsack}
& Explicit-origin & \textbackslash{}  & $43.12$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & \textbf{\textbf{42.42}}  & $41.47$ & $3.88$  & $4.24$&$0.19$&$0.72$&$29.56$&$31.34$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{43.17}} & $2.64$  & $2.54$& $0.37$  & $1.33$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Capacitated Warehouse Location}
& Explicit-origin & \textbackslash{}  & $31.37$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $25.49$  & $30.39$ & $0.00$  &$ 0.00$&$1.96$&$0.00$&\textbf{\textbf{53.92}}&$16.67$  \\
& Implicit-disorder & \textbackslash{}  &\textbf{\textbf{ 41.10}} & $2.35$  & $0.59$& $0.00$  & $1.10$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{2D-cutting Packing}
& Explicit-origin & \textbackslash{}  & $83.33$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $77.78$  & \textbf{\textbf{83.33}} & $16.67$  & $11.11$ & $0.00$ & $0.00$ & $38.89$ & $50.00$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{72.41}} & $0.00$  & $0.00$ & $0.00$  & $0.00$ & \textbackslash{}  & \textbackslash{}  \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[ht]
\centering
\caption{AR Task Performance Comparison}
\label{AR}
\resizebox{\textwidth}{!}{ % 使用 \resizebox 来调整表格大小
\begin{tabular}{llcccccccc}
\toprule
\multirow{2}{*}{Task} & \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{GPT-4o-mini} & \multicolumn{2}{c}{LLAMA3-8B} & \multicolumn{2}{c}{ORLM} & \multicolumn{2}{c}{DeepSeek-R1}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
 & & PoT & PoT+CoT & PoT & PoT+CoT &PoT & PoT+CoT &PoT & PoT+CoT \\
\midrule

\multirow{3}{*}{Assignment} 
& Explicit-origin & \textbackslash{}  & $0.00$ & \textbackslash{}   &  \textbackslash{} &  \textbackslash{} &  \textbackslash{} &  \textbackslash{} &  \textbackslash{}\\
& Implicit-origin & $4.41$  & \textbf{\textbf{10.00}} & $2.27$  & $5.00$ &$0.00$&$0.00$&$8.33$&$6.67$ \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{11.11}} & $0.00$  & $4.63$& $0.00$  & $0.93$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{1D-Binpacking}
& Explicit-origin & \textbackslash{}  & $10.85$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $5.94$  & $4.79$ & $6.04$  & $1.25$&$0.62$&$0.00$&$9.65$&\textbf{\textbf{10.07}}  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{4.48}} & $0.56$  & $1.72$ & $0.44$  & $0.54$& \textbackslash{}  & \textbackslash{} \\
\cmidrule(lr){1-10}

\multirow{3}{*}{Crew-scheduling}
& Explicit-origin & \textbackslash{}  & $0.00$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $1.33$  & $0.00$ & $0.00$  & $0.00$&$0.00$&$0.00$& \textbf{\textbf{27.33}} & $25.00$  \\
& Implicit-disorder & \textbackslash{}  & $0.00$ & $0.00$  & $0.00$& \textbf{\textbf{21.54}}  & $0.00$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{Steiner}
& Explicit-origin & \textbackslash{}  & $7.46$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $6.84$  & $7.24$ & $2.02$  & $1.63$&$0.20$&$0.00$& \textbf{\textbf{75.52}}& $6.47$  \\
& Implicit-disorder & \textbackslash{}  & $0.37$ & $0.41$  & \textbf{\textbf{1.10}}& $0.05$  & $0.26$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{UBQP}
& Explicit-origin & \textbackslash{}  & 0.74 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $0.00$  & $0.75$ &$ 0.74$  & $0.74$&$0.00$&$0.74$& \textbf{\textbf{3.70}}&$2.22$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.57}} & $0.44$  & $0.00$& $0.00$  & $0.44$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{CVRP}
& Explicit-origin & \textbackslash{}  & $3.11$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $5.41$  & $3.59$ & $0.00 $ & $0.00$ & $0.00$ & $0.00$& \textbf{\textbf{6.15}}&$2.69$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{3.14}} & $0.10$  & $0.00$& $0.00$  & $0.10$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{MDVRP}
& Explicit-origin & \textbackslash{}  & $11.36$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $6.06$ & \textbf{\textbf{8.33}} & $0.00$  &$ 0.00$ & $0.00$ & $0.00$& $4.55$&$1.52$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{11.62}} & $1.01$  & $0.00$& $0.00$  & $0.00$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{PVRP}
& Explicit-origin & \textbackslash{}  & $3.97$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $10.32$  & $7.94$ & $0.00$  & $0.00$&$0.00$&$0.00$& \textbf{\textbf{11.90}}&$11.48$  \\
& Implicit-disorder & \textbackslash{}  &\textbf{\textbf{ 11.43}} & $0.00$  & $0.00$& $0.00$  & $0.00$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Aircraft Landing}
& Explicit-origin & \textbackslash{}  & $4.55$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $11.36$  & $4.55$ & $0.00$  &$0.00$&$0.00$&$0.00$& \textbf{\textbf{45.45}}& $0.00$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{5.68}} & $1.14$  & $0.00$& $0.00$  & $0.00$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Generalised Assignment}
& Explicit-origin & \textbackslash{}  & $22.78$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & \textbf{\textbf{12.22}}  & $11.67$ & $3.33$  &$2.78$&$0.56$&$0.56$& $8.00$&$11.54$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{23.00}} & $3.33$  & $2.33$& $0.67$  & $0.33$& \textbackslash{}  & \textbackslash{}  \\

\cmidrule(lr){1-10}
\multirow{3}{*}{Multi-dimensional Knapsack}
& Explicit-origin & \textbackslash{}  & $3.75$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $0.72$  & $0.59$ & $0.36$  & $0.27$&$0.00$&$0.00$& \textbf{\textbf{0.94}}& $0.00$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{1.09}} & $0.18$  & $0.15$& $0.00$  & $0.00$& \textbackslash{}  & \textbackslash{}  \\

\cmidrule(lr){1-10}
\multirow{3}{*}{Capacitated Warehouse Location}
& Explicit-origin & \textbackslash{}  & $5.88$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $0.00$  & $0.00$ & $0.00$  & $0.00$&$0.00$&$0.00$& \textbf{\textbf{11.76}}&$2.94$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{5.52}} & $0.59$  & $0.00$& $0.00$  & $0.00$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{2D-cutting Packing}
& Explicit-origin & \textbackslash{}  & 27.78 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $5.56$  &$ 11.11$ & $0.00$  & $0.00$ & $0.00$ & $0.00$& $16.67$&\textbf{\textbf{33.33}}  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{24.14}} & $0.00$  & $0.00$& $0.00$  & $0.00$& \textbackslash{}  & \textbackslash{}  \\

% 其余任务按相同模式添加...
\bottomrule
\end{tabular}
}
\end{table}


\begin{table}[ht]
\centering
\caption{MAPE Task Performance Comparison}
\label{MAPE}
\resizebox{\textwidth}{!}{ % 使用 \resizebox 来调整表格大小
\begin{tabular}{llcccccccc}
\toprule
\multirow{2}{*}{Task} & \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{GPT-4o-mini} & \multicolumn{2}{c}{LLAMA3-8B} & \multicolumn{2}{c}{ORLM} & \multicolumn{2}{c}{DeepSeek-R1}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
 & & PoT & PoT+CoT & PoT & PoT+CoT &PoT & PoT+CoT &PoT & PoT+CoT \\
\midrule

\multirow{3}{*}{Assignment} 
& Explicit-origin & \textbackslash{}  & - & \textbackslash{}   &  \textbackslash{} &  \textbackslash{} &  \textbackslash{} &  \textbackslash{} &  \textbackslash{}\\
& Implicit-origin & $1.969$  & $1.969$ & -  & $1.876$ &$0.00$&\textbf{\textbf{0.534}}& $1.847$&$1.944$ \\
& Implicit-disorder & \textbackslash{}  & $1.838$ & -  & $2.276$& -  & \textbf{\textbf{0.220}}& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{1D-Binpacking}
& Explicit-origin & \textbackslash{}  & $0.089$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $0.2284$  & \textbf{\textbf{0.092}} & $0.727$  & $0.691$ & $1.267$ &$1.182$& $0.249$& $0.292$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.181}} & $0.811$  & $0.539$ & $1.526$  & $1.839$& \textbackslash{}  & \textbackslash{} \\
\cmidrule(lr){1-10}

\multirow{3}{*}{Crew-scheduling}
& Explicit-origin & \textbackslash{}  & $1.694$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & -  & $0.801$ & $2.691$  & - & - & -& $0.671$& \textbf{\textbf{0.421}}  \\
& Implicit-disorder & \textbackslash{}  & $1.866$ & -  & -& \textbf{\textbf{0.973}}  & -& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{Steiner}
& Explicit-origin & \textbackslash{}  & $0.758$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $1.269$  & $0.704$ & $1.751$  & $1.548$&$1.895$ & - & \textbf{\textbf{0.033}} & $0.926$  \\
& Implicit-disorder & \textbackslash{}  & $1.474$ & \textbf{\textbf{1.345}}  & $1.677$& $2.095$  & $1.390$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{UBQP}
& Explicit-origin & \textbackslash{}  & $0.579$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $0.391$  & \textbf{\textbf{0.315}} & -  & $0.577$ & - & - & $0.347$& $0.459$ \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.336}} & $0.601$  & - & -  & -& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{CVRP}
& Explicit-origin & \textbackslash{}  & $0.428$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $0.887$  & $0.424$ & $3.429$  & - & - & -& $0.641$& \textbf{\textbf{0.083}}  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.722}} & -  & - & -  & -& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{MDVRP}
& Explicit-origin & \textbackslash{}  & $1.226$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $0.836$ & $0.719$ & -  & - & - & - & \textbf{\textbf{0.698}}& $0.975$  \\
& Implicit-disorder & \textbackslash{}  & $1.300$ & \textbf{\textbf{0.451}}  & - & -  & -& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{PVRP}
& Explicit-origin & \textbackslash{}  & $1.401$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $1.501$  & $0.884$ & -  & - & - & -& \textbf{\textbf{0.798}}& $1.086$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.887}} & $3.200$  & - & -  & -& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Aircraft Landing}
& Explicit-origin & \textbackslash{}  & - & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $3.187$  & - & -  &$1.774$&-&- & \textbf{\textbf{0.892}}& -  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.381}} & -  & - & -  & -& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Generalised Assignment}
& Explicit-origin & \textbackslash{}  & $1.371$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $1.053$  & $1.048$ & $0.741 $ & \textbf{\textbf{0.024}} &$0.437$&-& $0.543$&$0.606$  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.868}} & $2.397$  & $0.872$& -  & -& \textbackslash{}  & \textbackslash{}  \\

\cmidrule(lr){1-10}
\multirow{3}{*}{Multi-dimensional Knapsack}
& Explicit-origin & \textbackslash{}  & $4.387$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $1.776$  & $1.756$ & \textbf{\textbf{1.087}}  & $1.163$ & - & $2.068$&$ 2.236$& $2.345$  \\
& Implicit-disorder & \textbackslash{}  & $1.953$ & $1.800$  & $1.691$& \textbf{\textbf{0.453}}  & -& \textbackslash{}  & \textbackslash{}  \\

\cmidrule(lr){1-10}
\multirow{3}{*}{Capacitated Warehouse Location}
& Explicit-origin & \textbackslash{}  & $0.842$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & -  & - & -  & - & - & -& \textbf{\textbf{0.016}}&$0.017 $ \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.064}} & $2.089$  & -& -  & -& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{2D-cutting Packing}
& Explicit-origin & \textbackslash{}  & $0.341$ & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $0.507$  & $0.353$ & $0.562$  & - & - & -& $0.776$&\textbf{\textbf{0.213}}  \\
& Implicit-disorder & \textbackslash{}  & \textbf{\textbf{0.576}} & -  & - & -  & -& \textbackslash{}  & \textbackslash{}  \\

% 其余任务按相同模式添加...
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[htbp]
\centering
\caption{Error Case Analysis in Common Research Problems}
\label{tab:error_analysis_en}
\begin{tabularx}{1.1\textwidth}{p{2cm}>{\raggedright\arraybackslash\hsize=1.2\hsize}X>{\raggedright\arraybackslash\hsize=0.7\hsize}X}
\toprule
\textbf{Task} & \textbf{Error} & \textbf{Reason} \\
\midrule
Assignment & cost\_matrix[i, j] = c& IndexError: index 3301 is out of bounds for axis 1 with size 3000 \\
1D-Binpacking & with open('data123.txt', 'r') as file:
\quad \quad \quad \quad \quad S = [float(line.strip()) for line in file]& ValueError: could not convert string to float: '[$\ldots$]' \\
\addlinespace
Crew-scheduling & cost[i][j] = c & IndexError: list assignment index out of range  \\
\addlinespace
Steiner & Timeout & TimeoutError: Operation Timed Out   \\
\addlinespace
UBQP & matrix[i][j] = c\_ij & IndexError: list assignment index out of range  \\
\addlinespace
CVRP & routing.AddDimensionWithVehicleCapacity(
    demand\_callback\_index,
    0,
    data,  
    True, 
    'Capacity'
) & TypeError: 'float' object cannot be interpreted as an integer \\
\addlinespace
MDVRP & 
    with open(filename, 'r') as f:   
\quad \quad \quad \quad \quad \quad data = f.read().strip().split('\textbackslash n') 
\quad \quad \quad \quad \quad \quad return [list(map(float, line.strip().split())) for line in data]
& ValueError: could not convert string to float: '[$\ldots$]' \\
\addlinespace
PVRP & routing = pywrapcp.RoutingModel(n\_nodes, num\_vehicles, depot\_index) & TypeError: Wrong number or type of arguments for overloaded function 'new\_RoutingModel'. \\
\addlinespace
Aircraft Landing & model += land\_time[i] $\geq$ land\_time[j] + sep\_matrix[j][i] - M * (before + (1 - same\_rw))) & SyntaxError: unmatched ')' \\
\addlinespace
Generalised Assignment & prob += lpSum(p[i][j] * x[i][j] for i in bins for j in items) & IndexError: list index out of range \\
\addlinespace
Multi-dimensional Knapsack & 
with open('data1.json', 'r') as f:
\quad\quad \quad \quad \quad \quad c = list(map(float, f.read().strip().split()))& ValueError: could not convert string to float: '[$\ldots$]'  \\
\addlinespace
Capacitated Warehouse Location & assert len(F) == 25 and len(d) == 50 and len(K) == 25 and len(c) == 25, 'Data dimensions incorrect' & AssertionError: Data dimensions incorrect \\
\addlinespace
2D-cutting Packing & l = int(float(l\_str)) &ValueError: could not convert string to float: '[$\ldots$]'  \\
\addlinespace
\bottomrule
\end{tabularx}
\end{table}

\begin{table}[ht]
\centering
\caption{Timeout Task Performance Comparison}
\label{timeout}
\resizebox{\textwidth}{!}{ % 使用 \resizebox 来调整表格大小
\begin{tabular}{llcccccccc}
\toprule
\multirow{2}{*}{Task} & \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{GPT-4o-mini} & \multicolumn{2}{c}{LLAMA3-8B} & \multicolumn{2}{c}{ORLM} & \multicolumn{2}{c}{DeepSeek-R1}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
 & & PoT & PoT+CoT & PoT & PoT+CoT &PoT & PoT+CoT &PoT & PoT+CoT \\
\midrule

\multirow{3}{*}{Assignment} 
& Explicit-origin & \textbackslash{}  & 0.00 & \textbackslash{}   &  \textbackslash{} &  \textbackslash{} &  \textbackslash{} &  \textbackslash{} &  \textbackslash{}\\
& Implicit-origin & 0.00  & 0.00 & 0.00  & 3.33 &0.00&1.67& 1.67 &$\overline{\textbf{11.67}}$ \\
& Implicit-disorder & \textbackslash{}  & $\underline{\textbf{0.93}}$ & 1.85  & 1.85& 1.85  & $\overline{\textbf{2.78}}$& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{1D-Binpacking}
& Explicit-origin & \textbackslash{}  & 11.55 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & 15.00  & 4.62 & 6.04  & $\underline{\textbf{0.94}}$ & 2.92 &4.17& $\overline{\textbf{16.74}}$ &15.10  \\
& Implicit-disorder & \textbackslash{}  & 0.80 & $\overline{\textbf{1.49}}$  & 0.77 & $\underline{\textbf{0.63}}$  & 1.08& \textbackslash{}  & \textbackslash{} \\
\cmidrule(lr){1-10}

\multirow{3}{*}{Crew-scheduling}
& Explicit-origin & \textbackslash{}  & 12.67 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $\overline{\textbf{20.67}}$  & 16.00 & 1.33  & 3.33 & $\underline{\textbf{0.67}}$ & 3.33& 9.33 &9.26  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{24.39}}$ & $\underline{\textbf{0.40}}$  & 0.80& 13.85  & 1.20& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{Steiner}
& Explicit-origin & \textbackslash{}  & 10.15 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $\overline{\textbf{10.41}}$  & 5.92 & 9.96  & 7.76&2.35&0.92& $\underline{\textbf{0.78}}$ &1.56  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{22.79}}$ & $\underline{\textbf{1.63}}$  & 6.23& 1.33  & 2.76& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{UBQP}
& Explicit-origin & \textbackslash{}  & 35.56 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $\overline{\textbf{64.44}}$  & 21.64 & 2.22  & $\underline{\textbf{0.74}}$ & $\underline{\textbf{0.74}}$ & 2.96& 31.85 &4.44  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{21.26}}$ & 0.00  & 0.00& 0.00  & 1.78& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{CVRP}
& Explicit-origin & \textbackslash{}  & 1.33 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & 20.78  & 6.37 & 0.16  & 0.00 & 0.98 & 0.16& $\overline{\textbf{24.82}}$ &4.57  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{8.33}}$ & 1.27  & $\underline{\textbf{0.20}}$& 0.78  & 1.08& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{MDVRP}
& Explicit-origin & \textbackslash{}  & 3.03 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & $\overline{\textbf{4.55}}$ & 3.03 & 0.76  & 0.76 & 0.00 & 0.00& 0.00 &1.52  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{3.54}}$ & 1.01  & 0.51& 0.51  & 0.00& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{PVRP}
& Explicit-origin & \textbackslash{}  & 11.90 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & 11.90  & 11.11 & 0.79  & 0.00 & 0.79 & 0.00& 8.73 &$\overline{\textbf{14.75}}$  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{12.86}}$ & 1.43  & 0.00& 0.48  & 0.48& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Aircraft Landing}
& Explicit-origin & \textbackslash{}  & 0.00 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & 9.09  & 0.00 & 0.00  &0.00&0.00&0.00& $\overline{\textbf{18.18}}$ &9.09  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{7.95}}$ & 0.00  & 1.14& 0.00  & 0.00& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}
\multirow{3}{*}{Generalised Assignment}
& Explicit-origin & \textbackslash{}  & 0.00 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & 1.11  & $\overline{\textbf{2.78}}$ & 0.00  & 0.00 &0.56&0.56& 0.00 &0.00  \\
& Implicit-disorder & \textbackslash{}  & 1.33 & 0.00  & 0.00& $\overline{2.00}$  & 0.00& \textbackslash{}  & \textbackslash{}  \\

\cmidrule(lr){1-10}
\multirow{3}{*}{Multi-dimensional Knapsack}
& Explicit-origin & \textbackslash{}  & 5.63 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & 8.66  & 15.59 & 0.99  & 0.90 & 0.85 & $\underline{\textbf{0.72}}$& 38.36 &$\overline{\textbf{57.71}}$  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{19.95}}$ & 0.35  & $\underline{\textbf{0.15}}$& 0.37  & 0.20& \textbackslash{}  & \textbackslash{}  \\

\cmidrule(lr){1-10}
\multirow{3}{*}{Capacitated Warehouse Location}
& Explicit-origin & \textbackslash{}  & 2.94 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & 0.00  & 0.00 & 0.00  & 0.00 & 0.00 & 0.00& 0.00 &$\overline{\textbf{0.98}}$  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{3.07}}$ & 0.00  & 0.00& 0.59  & 0.00& \textbackslash{}  & \textbackslash{}  \\
\cmidrule(lr){1-10}

\multirow{3}{*}{2D-cutting Packing}
& Explicit-origin & \textbackslash{}  & 5.56 & \textbackslash{}  & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{} & \textbackslash{}  \\
& Implicit-origin & 0.00  & 5.56 & 0.00  & 0.00 & 0.00 & 0.00& 11.11 &$\overline{\textbf{38.89}}$  \\
& Implicit-disorder & \textbackslash{}  & $\overline{\textbf{6.90}}$ & 0.00  & 0.00& 0.00  & 0.00& \textbackslash{}  & \textbackslash{}  \\

% 其余任务按相同模式添加...
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Performance Effectiveness of Different Problems}
    \footnotesize
    \begin{tabular}{@{\extracolsep{\fill}} l p{5cm} p{5cm} @{}}
        \toprule
        \textbf{Status} & \textbf{Status Descriptions}& \textbf{Problems} \\ 
        \midrule
        Worsened & Disordered datasets are slightly inferior &1D-Binpacking, Crew-scheduling, CVRP \\ \midrule
        Significantly Worsened & Disordered datasets are greatly inferior &Steiner, UBQP \\ \midrule
        Improved & Disordered datasets are slightly superior &Assignment, MDVRP, Aircraft Landing, Multi-dimensional Knapsack \\ \midrule
        Significantly Improved & Disordered datasets are greatly superior  &PVRP, Generalised Assignment, Capacitated Warehouse Location, 2D-Cutting Packing-Constrained Guillotine \\ 
        \bottomrule
    \end{tabular}
    \label{tab:problem_changes}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Assignment Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 0 & 9.52 & 0 & 0 &80.95 & 0 & 4.76 & 4.76 & 0 & 0 & 0 \\ 
        \hdashline
        GPT-4o-mini, PoT, Implicit & 24.24 & 3.03 & 0 & 0 & \textbf{57.58} & 0 & 0 & 12.12 & 3.03 & 0 & 0 \\ 
        GPT-4o-mini, PoT+CoT, Implicit & 19.57 & 2.17 & 0 & 0 & \textbf{67.39} & 0 & 0 & 10.87 & 0 & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 0 & 0 & 0 & 0 & \textbf{28.89} & 0 & 0 & 0 & 2.22 & 0 & 0 \\
        LLAMA3-8B, PoT, Implicit & 2.22 & 0 & 0 & 4.44 & \textbf{53.33} & 4.44 & 0 & 4.44 & 8.89 & 0 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 9.80 & 0 & 1.96 & 0 & \textbf{35.29} & 0 & 0 & 3.92 & 5.88 & 0 & 0 \\ 
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 22.22 & 3.03 & 1.01 & 5.05 & \textbf{53.54} & 1.01 & 0 & 3.03 & 4.04 & 0 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 3.70 &0&0&3.70& \textbf{55.56} & 1.23 & 0 & 3.70 & 12.35 & 1.23 & 0  \\
        ORLM, PoT, Implicit(\%) & 1.03 & 0.69 & 0 & 3.10 & \textbf{5.52} & 3.10 & 0.69 & 7.24 & 1.03 & 0.34 & 0 \\
        ORLM, PoT+CoT, Implicit(\%) & 3.32 & 1.85 & 0 & 3.32 & 8.86 & 4.06 & 0.37 & \textbf{9.59} & 4.06 & 0.74 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 2.69 & 2.31 & 0 & 3.85 & 5.96 & 4.62 & 0.38 & \textbf{7.88} & 1.92 & 0.58 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 2.85 & 1.63 & 0.20 & 3.25 & \textbf{8.33} & 3.05 & 0.00 & 6.71 & 3.05 & 0.41 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 0 & 0 & 0 & 0 & \textbf{50} & 0 & 0 & 0 & 0 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & 9.09 & 0 & 0 & 0 & \textbf{50} & 0 & 0 & 0 & 0 & 0 & 0 \\
          
        \bottomrule
    \end{tabular}}
    \label{tab2}
\end{table}

\begin{table}[ht]
    \centering
    \caption{1D-Binpacking Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 0 & 0 & 0 & 0 & \textbf{80.95} & 9.52 & 0 & 0 & 4.76 & 0 & 0 \\
        \hdashline
        GPT-4o-mini, PoT, Implicit & 4.23 & 0 & 0 & 0.39 & \textbf{38.58} & 0.16 & 0.08 & 0.16 & 1.49 & 0.39 & 0 \\ 
        GPT-4o-mini, PoT+CoT, Implicit & 3.23 & 0 & 0 & 0 & \textbf{93.55} & 0 & 0 & 0 & 3.23 & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 8.47 & 0 & 0 & 0.13 & 91.27 & 0 & 0 & 0 & 0.13 & 0 & 0 \\
        LLAMA3-8B, PoT, Implicit & 7.19 & 5.12 & 0.12 & 11.81 & \textbf{59.44} & 2.07 & 2.19 & 4.51 & 7.31 & 0.24 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 1.24 & 0 & 0.08 & 1.17 & \textbf{56.45} & 0.86 & 0.47 & 2.18 & 1.32 & 0.16 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 1.70 & 10.21 & 0 & 2.55 & \textbf{70.64} & 2.13 & 1.70 & 5.53 & 4.26 & 1.28 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 1.40 & 3.85 & 0 & 0.87 & \textbf{68.85} & 1.40 & 0.44 & 1.75 & 1.92 & 0.17 & 0 \\
        ORLM, PoT, Implicit(\%) & 17.26 & 5.58 & 0 & 10.66 & \textbf{28.43} & 12.69 & 0 & 17.77 & 7.11 & 0.51 & 0 \\ 
        ORLM, PoT+CoT, Implicit(\%) & 2.98 & 1.75 & 0.07 & 3.13 & 4.66 & 3.13 & 0.15 & \textbf{6.11} & 2.40 & 0.44 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 14.50 & 4.46 & 0 & 12.27 & 14.87 & 14.13 & 1.12 & \textbf{30.48} & 7.06 & 1.12 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 8.02 & \textbf{31.28} & 0 & 9.63 & 8.29 & 9.36 & 0 & 27.54 & 4.01 & 1.87 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 15.94 & 0 & 0 & 0 & \textbf{28.87} & 0.23 & 0.69 & 0.46 & 0 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & \textbf{29.23} & 2.31 & 0 & 0.77 & 22.31 & 0.77 & 0 & 0 & 0.77 & 0.77 & 0 \\
         
        \bottomrule
    \end{tabular}}
    \label{tab4}
\end{table}

\begin{table}[htbp!]
    \centering
    \caption{Crew-scheduling Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & \textbf{30.77} & 14.62 & 2.31 & 7.69 & 26.92 & 3.85 & 4.62 & 2.31 & 5.38 & 0.77 & 0.77 \\ 
        \hdashline
        GPT-4o-mini, PoT, Implicit & 46.4 & 3.6 & 0.4 & 0.8 & \textbf{35.2} & 0.4 & 0 & 4.4 & 8 & 0.4 & 0.4 \\ 
        GPT-4o-mini, PoT+CoT, Implicit & \textbf{48.06} & 6.20 & 0 & 2.71 & 31.78 & 1.94 & 0.39 & 6.20 & 2.33 & 0 & 0.39 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 33.67 & 0 & 0.80 & 0.80 & \textbf{35.46} & 0.60 & 0.20 & 0.20 & 1.39 & 0 & 0 \\  
        LLAMA3-8B, PoT, Implicit & 19.61 & 0 & 0 & 5.23 & \textbf{25.49} & 0.65 & 3.92 & 9.80 & 11.76 & 0.65 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 30.47 & 0.78 & 0.78 & 5.47 & \textbf{38.28} & 1.56 & 0.78 & 16.41 & 4.69 & 0.78 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 28.46 & 0 & 0 & 4.88 & \textbf{32.52} & 3.25 & 1.63 & 12.60 & 6.50 & 1.63 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 22.89 & 0 & 0 & 3.21 & \textbf{35.34} & 0 & 1.61 & 12.05 & 10.84 & 2.01 & 0 \\
        ORLM, PoT, Implicit(\%) & 11.76 & 0 & 0 & 17.65 & 11.76 & 11.76 & 0 & \textbf{47.06} & 0 & 0 & 0 \\ 
        ORLM, PoT+CoT, Implicit(\%) & 7.05 & 2.12 & 0.14 & 7.90 & 9.31 & 4.80 & 0.71 & \textbf{10.72} & 3.67 & 0.42 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & \textbf{34.78} & 2.17 & 3.62 & 0.72 & 0.72 & 0.72 & 0.72 & 2.90 & 7.25 & 10.87 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 2.62 & 4.84 & 0 & 5.00 & 3.44 & 2.95 & 0.25 & \textbf{9.34} & 2.79 & 0.49 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & \textbf{59.78} & 3.26 & 0 & 0 & 1.09 & 2.17 & 1.09 & 5.43 & 6.52 & 20.65 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & \textbf{32.89} & 0.67 & 0.67 & 0.67 & 0 & 4.03 & 2.01 & 4.03 & 9.40 & 12.08 & 0 \\
        \bottomrule
    \end{tabular}}
    \label{tab6}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Steiner Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 0 & 0 & 0 & 0 & \textbf{85} & 0 & 0 & 0 & 15 & 0 & 0 \\ 
        \hdashline
        GPT-4o-mini, PoT, Implicit & 4.14 & 3.45 & 0 & 2.76 & \textbf{12.87} & 2.30 & 4.37 & 3.91 & 12.18 & 0.92 & 0.23 \\ 
        GPT-4o-mini, PoT+CoT, Implicit & 8.55 & 1.32 & 0 & 8.55 & 7.89 & 1.32 & 2.63 & 29.61 & \textbf{40.13} & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 0.92 & 0 & 0 & 0.56 & 1.34 & 0.21 & 0.28 & 1.41 & \textbf{3.39} & 0.07 & 0 \\
        LLAMA3-8B, PoT, Implicit & 7.03 & 0.41 & 0 & 8.24 & 8.92 & 2.16 & 0.41 & 8.51 & \textbf{27.57} & 0.14 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 4.51 & 0.16 & 0 & 8.09 & 7.78 & 1.17 & 3.42 & 9.34 & \textbf{21.32} & 0 & 0 \\ 
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 13.82 & 5.69 & 0 & 5.69 & 8.94 & 1.63 & 1.63 & \textbf{39.84} & 22.76 & 0 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 11.09 & 0.33 & 0.76 & 14.02 & 14.24 & 1.85 & 6.63 & 13.48 & \textbf{37.28} & 0.33 & 0 \\
        ORLM, PoT, Implicit(\%) & 1.39 & 0 & 0 & 3.73 & 3.36 & 2.12 & 0.29 & \textbf{5.12} & 3.00 & 1.10 & 0 \\ 
        ORLM, PoT+CoT, Implicit(\%) & 6.16 & 0.47 & 0 & 23.70 & 11.85 & 5.69 & 1.42 & \textbf{36.49} & 11.37 & 2.84 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 1.24 & 0.59 & 0 & 2.49 & 1.98 & 1.39 & 0.15 & \textbf{8.71} & 2.41 & 0.73 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 1.68 & 0.66 & 0 & 4.52 & 3.28 & 1.60 & 0.22 & \textbf{8.97} & 3.65 & 0.95 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 0.23 & 0 & 0 & 1.16 & 2.55 & 0 & 0 & \textbf{6.96} & 0.46 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & 1.35 & 1.35 & 1.35 & 2.70 & 16.22 & 2.70 & 0 & \textbf{40.54} & 5.41 & 0 & 0 \\
         
        \bottomrule
    \end{tabular}}
    \label{tab8}
\end{table}

\begin{table}[ht]
    \centering
    \caption{UBQP Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 25.53 & 8.51 & 0 & 2.13 & \textbf{53.19} & 2.13 & 0 & 4.26 & 2.13 & 2.13 & 0 \\ 
        \hdashline
        GPT-4o-mini, PoT, Implicit & \textbf{62.04} & 10.22 & 0.73 & 1.46 & 23.36 & 0.73 & 0 & 0.73 & 0.73 & 0 & 0 \\ 
        GPT-4o-mini, PoT+CoT, Implicit & \textbf{47.83} & 17.39 & 0 & 1.74 & 32.17 & 0.87 & 0 & 0 & 0 & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 29.04 & 0 & 0 & 0 & 0.60 & \textbf{39.82} & 0.30 & 0 & 0.30 & 0.30 & 0 \\
        LLAMA3-8B, PoT, Implicit & 18.18 & 0 & 0 & 1.65 & \textbf{41.32} & 0.83 & 2.48 & 6.61 & 12.40 & 0 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 17.39 & 0 & 0 & 3.73 & \textbf{28.57} & 2.48 & 0 & 1.24 & 14.29 & 1.24 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 18.69 & 1.52 & 0.51 & 2.02 & \textbf{56.06} & 2.53 & 0.51 & 0.51 & 8.08 & 1.01 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 14.29 & 1.38 & 0 & 1.84 & \textbf{57.60} & 2.76 & 0.46 & 4.61 & 5.53 & 0.46 & 0 \\
        ORLM, PoT, Implicit(\%) & 0.92 & 0.15 & 0.15 & 1.99 & 3.21 & 0.76 & 0 & \textbf{7.80} & 1.38 & 0.46 & 0 \\  
        ORLM, PoT+CoT, Implicit(\%) & 6.16 & 1.11 & 0.47 & 6.79 & \textbf{16.59} & 4.27 & 0.32 & 10.43 & 6.00 & 2.21 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 1.99 & 0.27 & 0 & 1.72 & 3.70 & 1.17 & 0.09 & \textbf{6.68} & 1.36 & 0.27 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 3.63 & 1.24 & 0.10 & 4.88 & 9.85 & 4.11 & 0.48 & \textbf{10.61} & 3.35 & 1.43 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & \textbf{34.74} & 0 & 5.26 & 0 & 0 & 0 & 0 & 1.05 & 1.05 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & \textbf{60.66} & 1.64 & 0 & 3.28 & 0 & 0 & 0 & 11.48 & 0 & 0 & 0 \\
        \bottomrule
    \end{tabular}}
    \label{tab10}
\end{table}

\begin{table}[ht]
    \centering
    \caption{CVRP Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 10.29 & 15.04 & 1.06 & 2.90 & 7.65 & 12.93 & 13.46 & 3.17 & 16.36 & \textbf{16.89} & 0.26 \\ 
        \hdashline
        GPT-4o-mini, PoT, Implicit & 8.52 & 0 & 0.14 & 2.79 & \textbf{34.43} & 3.21 & 19.97 & 0.77 & 4.61 & 2.86 & 0.21 \\ 
        GPT-4o-mini, PoT+CoT, Implicit & 2.87 & 1.91 & 0.64 & 1.59 & 13.69 & 14.33 & \textbf{27.39} & 3.18 & 16.24 & 18.15 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 4.98 & 0.09 & 0.27 & 2.22 & 18.84 & 13.07 & \textbf{22.84} & 3.47 & 15.82 & 18.40 & 0 \\
        LLAMA3-8B, PoT, Implicit & 2.51 & 0 & 0 & 1,76 & 7.40 & 5.27 & 6.52 & \textbf{17.69} & 4.77 & 0.50 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 2.30 & 0.27 & 0 & 4.47 & 14.88 & 9.88 & 7.44 & \textbf{21.65} & 10.56 & 4.06 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 4.31 & 0.49 & 0.10 & 4.40 & 12.62 & 12.82 & 12.04 & \textbf{19.57} & 14.38 & 3.03 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 2.96 & 0.10 & 0 & 4.21 & 10.42 & 17.59 & 8.99 & \textbf{24.86} & 16.63 & 2.87 & 0 \\
        ORLM, PoT, Implicit(\%) & 3.20 & 2.28 & 0 & 20.09 & 12.33 & 11.42 & 12.79 & \textbf{25.57} & 9.13 & 3.20 & 0 \\ 
        ORLM, PoT+CoT, Implicit(\%) & 3.17 & 3.49 & 0 & 10.79 & 14.29 & 8.89 & 7.62 & \textbf{42.54} & 5.40 & 3.81 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 1.71 & 7.17 & 0 & 17.75 & 10.92 & 8.53 & 6.48 & \textbf{35.84} & 8.87 & 2.73 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 0.44 & 1.53 & 0 & 4.09 & 2.04 & 1.68 & 1.17 & \textbf{12.92} & 1.46 & 1.82 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 0.39 & 0 & 0 & 0.59 & 10.39 & 9.41 & 20.98 & 9.22 & \textbf{24.71} & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & 1.55 & 0.62 & 2.17 & 2.48 & 10.53 & 10.84 & 2.48 & 12.07 & \textbf{31.89} & 0 & 0 \\
        \bottomrule
    \end{tabular}}
    \label{tab12}
\end{table}

\begin{table}[ht]
    \centering
    \caption{MDVRP Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & \textbf{29.02} & 6.70 & 0 & 11.61 & 16.07 & 9.38 & 6.25 & 4.91 & 9.38 & 6.70 & 0 \\
        \hdashline
        GPT-4o-mini, PoT, Implicit & 4.05 & 5.41 & 0.68 & 7.43 & 10.81 & 8.78 & 10.14 & 11.49 & \textbf{37.16} & 4.05 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit & 14.12 & 4.71 & 0 & 5.88 & 13.53 & 0 & 4.71 & 23.53 & \textbf{30.59} & 1.76 & 1.18 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 5.05 & 0 & 0 & 7.41 & 8.75 & 0.67 & 2.69 & 2.36 & \textbf{19.53} & 2.69 & 0.67 \\
        LLAMA3-8B, PoT, Implicit & 7.48 & 0 & 0 & 14.97 & 5.44 & 5.44 & 5.44 & \textbf{23.81} & 3.40 & 0.68 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 0.95 & 0 & 0 & 10.48 & 5.24 & 7.14 & 1.43 & \textbf{12.86} & 9.52 & 1.90 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 7.81 & 0 & 0 & 9.90 & \textbf{23.44} & 6.77 & 5.21 & 15.63 & 14.58 & 5.21 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 2.51 & 0 & 0 & 11.06 & 17.59 & 7.54 & 4.02 & \textbf{24.12} & 14.57 & 2.01 & 0 \\
        ORLM, PoT, Implicit(\%) & 0.31 & 0.15 & 0 & 2.76 & 1.07 & 0.46 & 0.31 & \textbf{6.43} & 1.99 & 0.61 & 0 \\ 
        ORLM, PoT+CoT, Implicit(\%) & 0.61 & 1.23 & 0 & 3.53 & 1.07 & 1.07 & 0.92 & \textbf{6.29 }& 3.53 & 0.92 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 0.92 & 1.23 & 0 & 2.66 & 1.13 & 1.13 & 0.20 & \textbf{6.45} & 2.46 & 0.31 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 0.31 & 1.34 & 0 & 2.99 & 1.44 & 0.93 & 0.31 & \textbf{5.57} & 2.68 & 0.52 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 6.54 & 1.87 & 0.93 & 1.87 & \textbf{29.91} & 5.61 & 2.80 & 9.35 & 13.08 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & \textbf{39.61} & 0.48 & 0 & 1.45 & 21.26 & 9.66 & 3.38 & 11.59 & 12.56 & 0.00 & 0 \\
         
        \bottomrule
    \end{tabular}}
    \label{tab14}
\end{table}

\begin{table}[ht]
    \centering
    \caption{PVRP Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 2.14 & 0 & 0 & 8.02 & 3.74 & 5.88 & \textbf{32.09} & 3.21 & 5.35 & 6.42 & 2.67 \\
        \hdashline
        GPT-4o-mini, PoT, Implicit & 7.97 & 3.62 & 0 & 9.42 & 10.87 & 5.07 & \textbf{18.84} & 18.11 & 18.12 & 7.97 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit & 5.47 & 2.34 & 0 & 10.94 & \textbf{33.59} & 2.34 & 21.88 & 7.03 & 11.72 & 3.13 & 1.56 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 3.02 & 0 & 0.43 & 5.17 & 10.78 & 1.72 & 5.60 & 4.31 & \textbf{11.64} & 5.60 & 0.43 \\
        LLAMA3-8B, PoT, Implicit & 1.66 & 0 & 0 & 5.52 & 3.31 & 2.76 & 4.97 & \textbf{22.10} & 4.97 & 1.10 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 2.11 & 0 & 0 & 6.75 & 2.95 & 5.91 & 3.38 & \textbf{15.61} & 8.44 & 1.69 & 0 \\ 
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 5.09 & 0 & 0 & 12.04 & 10.19 & 9.72 & 6.48 & \textbf{25.00} & 17.59 & 0.46 & 0.46 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 3.65 & 0 & 0 & 12.33 & 11.87 & 5.48 & 8.22 & \textbf{22.37} & 12.79 & 0.46 & 0 \\
        ORLM, PoT, Implicit(\%) & 0.16 & 0.48 & 0 & 2.75 & 0 & 0.48 & 0.16 & \textbf{3.39} & 0.81 & 0.81 & 0 \\ 
        ORLM, PoT+CoT, Implicit(\%) & 0.64 & 0.48 & 0 & 2.56 & 0.64 & 1.76 & 0.48 & 4.33 & \textbf{2.72} & 0.80 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 0.29 & 0.87 & 0 & 2.50 & 0.77 & 1.06 & 0.58 & \textbf{6.65} & 2.02 & 0.48 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 0.68 & 0.39 & 0 & 3.29 & 0.58 & 1.06 & 0.97 & \textbf{6.57} & 1.93 & 0.19 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 0 & 0 & 0 & 4.59 & \textbf{24.77} & 5.50 & 4.59 & 10.09 & 16.51 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & 1.14 & 0 & 1.14 & 3.41 & 14.77 & 1.14 & 4.55 & \textbf{15.91} & 10.23 & 0 & 0 \\
        \bottomrule
    \end{tabular}}
    \label{tab16}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Aircraft Landing Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 13 & 4 & 0 & 1 & \textbf{37} & 9 & 0 & 1 & 34 & 0 & 1 \\
        \hdashline
        GPT-4o-mini, PoT, Implicit & 3.33 & 0 & 0 & 3.33 & 30 & 0 & 0 & 10 & \textbf{53.33} & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit & 2.60 & 0 & 0 & 6.49 & \textbf{38.96} & 0 & 0 & 11.69 & \textbf{38.96} & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 0.74 & 0 & 0 & 2.22 & \textbf{34.81} & 0.74 & 0 & 0 & 10.37 & 0 & 0.74 \\ 
        LLAMA3-8B, PoT, Implicit & 2.38 & 0 & 0 & 2.38 & \textbf{59.52} & 0 & 0 & 4.76 & 7.14 & 0 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 1.37 & 0 & 0 & 2.74 & \textbf{31.51} & 0 & 1.37 & 2.74 & 9.59 & 0 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 5.56 & 0 & 0 & 9.72 & \textbf{55.56} & 2.78 & 1.39 & 2.78 & 13.89 & 2.78 & 0  \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 3.57 & 0 & 0 & 7.14 & \textbf{40.48} & 1.19 & 7.14 & 14.29 & 15.48 & 1.19 & 0 \\
        ORLM, PoT, Implicit(\%) & 0.93 & 1.40 & 0 & 2.80 & 4.21 & 1.40 & 0.93 & \textbf{8.41} & 4.21 & 0.47 & 0 \\
        ORLM, PoT+CoT, Implicit(\%) & 0 & 0 & 0 & 4.65 & 1.86 & 2.33 & 1.40 & \textbf{6.05} & 3.72 & 0.47 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 2.30 & 1.15 & 0 & 2.99 & 3.45 & 1.38 & 1.15 & \textbf{7.36} & 1.38 & 0.46 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 0.70 & \textbf{7.96} & 0 & 3.04 & 1.87 & 0.23 & 0.23 & 3.98 & 0.94 & 0 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 9.52 & 0 & 0 & 0 & \textbf{40.48} & 0 & 0 & 16.67 & 7.14 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & \textbf{50} & 0 & 0 & 0 & 37.5 & 0 & 0 & 10.94 & 1.56 & 0 & 0 \\
          
        \bottomrule
    \end{tabular}}
    \label{tab18}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Generalised Assignment Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & \textbf{60.80} & 8.52 & 0 & 5.11 & 7.95 & 3.98 & 7.39 & 0.57 & 2.27 & 2.27 & 1.14 \\ 
        \hdashline
        GPT-4o-mini, PoT, Implicit & 12.98 & 2.67 & 0.38 & 15.27 & 16.79 & 0.38 & 1.15 & 3.82 & \textbf{44.27} & 0.38 & 1.91 \\
        GPT-4o-mini, PoT+CoT, Implicit & 9.15 & 5.23 & 0 & 14.38 & \textbf{29.74} & 1.30 & 15.03 & 2.29 & 21.57 & 1.31 & 0.33 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 3.85 & 3.40 & 0 & \textbf{20.41} & 19.50 & 2.27 & 0 & 2.04 & 3.17 & 0.23 & 0.91 \\
        LLAMA3-8B, PoT, Implicit & 13.41 & 8.94 & 0 & 1.68 & \textbf{36.87} & 5.03 & 6.15 & 15.08 & 3.35 & 0 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 17.95 & 1.03 & 0 & 5.13 & \textbf{24.62} & 4.10 & 4.62 & 15.38 & 5.64 & 0.51 & 0 \\ 
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 9.25 & 8.90 & 0 & 7.12 & \textbf{44.48} & 3.91 & 1.42 & 12.10 & 6.05 & 0.36 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 12.80 & 7.61 & 0 & 6.92 & \textbf{31.14} & 4.84 & 4.50 & 16.96 & 7.96 & 0 & 0 \\
        ORLM, PoT, Implicit(\%) & 1.15 & 0.46 & 0 & \textbf{4.70} & 4.36 & 3.90 & 0.46 & 3.21 & 4.36 & 0.69 & 0 \\
        ORLM, PoT+CoT, Implicit(\%) & 2.31 & 0.93 & 0 & 5.09 & 3.70 & 3.24 & 0.46 & \textbf{10.07} & 2.66 & 0.69 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 3.21 & 4.49 & 0 & 19.23 & 14.74 & 9.94 & 1.28 & \textbf{31.41} & 13.78 & 1.92 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 4.24 & 7.63 & 0 & 19.49 & 16.10 & 10.59 & 0 & \textbf{32.20} & 8.47 & 1.27 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & \textbf{41.67} & 0 & 0 & 0 & 15.15 & 0 & 0.76 & 2.27 & 40.15 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & \textbf{37.80} & 0 & 0 & 0 & 8.54 & 0 & 0 & 0 & 1.22 & 0 & 0 \\
        \bottomrule
    \end{tabular}}
    \label{tab20}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Multi-dimensional Knapsack Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 37.62 & 0.99 & 0 & 2.31 & \textbf{42.24} & 0.33 & 0 & 10.56 & 5.61 & 0.33 & 0 \\ 
        \hdashline
        GPT-4o-mini, PoT, Implicit & \textbf{26.28} & 1.53 & 0 & 2.04 & 52.04 & 0 & 0 & 0.77 & 17.09 & 0.26 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit & 22.61 & 1.01 & 0 & 2.76 & \textbf{52.26} & 0.98 & 0 & 1.26 & 19.10 & 0.25 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 17.59 & 0.08 & 0 & 2.65 & \textbf{44.28} & 0.30 & 0.23 & 0.76 & 16.53 & 0 & 0 \\ 
        LLAMA3-8B, PoT, Implicit & 6.58 & 0.12 & 0 & 1.85 & \textbf{75.98} & 2.08 & 0.23 & 8.31 & 4.73 & 0.12 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 6.41 & 0.38 & 0.13 & 2.14 & \textbf{73.99} & 3.77 & 0.25 & 6.66 & 6.03 & 0.25 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 4.16 & 0.13 & 0 & 0.76 & \textbf{48.42} & 2.40 & 0.13 & 10.47 & 2.90 & 0 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 4.87 & 0.23 & 0 & 0.93 & \textbf{54.87} & 2.09 & 0.58 & 6.26 & 6.38 & 0.35 & 0 \\
        ORLM, PoT, Implicit(\%) & 3.38 & 6.39 & 0 & 16.54 & \textbf{32.71} & 7.14 & 0.75 & 21.05 & 9.77 & 2.26 & 0 \\
        ORLM, PoT+CoT, Implicit(\%) & 4.22 & 5.84 & 0 & 9.42 & 31.82 & 5.52 & 0.65 & \textbf{33.77} & 6.17 & 2.60 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 3.66 & 6.50 & 0 &13.41 & 18.29 & 10.57 & 0.81 & \textbf{38.62} & 6.91 & 1.22 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 2.97 & 0.10 & 0 & 4.21 & 10.44 & 17.62 & 8.91 & \textbf{24.81} & 16.67 & 2.87 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 15.88 & 0 & 0 & 0 & \textbf{29.79} & 3.60 & 12.60 & 1.31 & 3.27 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & \textbf{16.22} & 0 & 0 & 0 & 29.73 & 0 & 0 & 0.34 & 0.68 & 0 & 0 \\
          
        \bottomrule
    \end{tabular}}
    \label{tab22}
\end{table}

\begin{table}[ht]
    \centering
    \caption{Capacitated warehouse location Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & \textbf{43.98} & 4.71 & 0.52 & 6.81 & 17.28 & 0 & 12.57 & 8.90 & 3.14 & 1.57 & 0.52 \\
        \hdashline
        GPT-4o-mini, PoT, Implicit & 23.51 & 0.37 & 0 & 3.36 & \textbf{66.79} & 0.37 & 0 & 0.37 & 5.22 & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit & \textbf{26.09} & 3.56 & 0 & 5.53 & 55.73 & 0.75 & 0.40 & 1.19 & 4.74 & 0.40 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 21.05 & 1.91 & 0 & 3.83 & \textbf{48.09} & 0.48 & 0 & 0.24 & 3.11 & 0.24 & 0 \\
        LLAMA3-8B, PoT, Implicit & 0 & 0 & 0 & 1.89 & \textbf{64.15} & 3.77 & 0.94 & 10.38 & 1.89 & 0 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 6.29 & 0 & 0 & 2.52 & \textbf{29.56} & 3.77 & 1.26 & 14.47 & 3.77 & 0 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 1.81 & 0 & 0 & 1.81 & \textbf{59.64} & 3.01 & 1.20 & 18.67 & 7.23 & 0 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 2.94 & 0 & \textbf{0} & 2.35 & \textbf{56.47} & 2.35 & 1.18 & 24.12 & 5.29 & 0.59 & 0 \\
        ORLM, PoT, Implicit(\%) & 1.03 & 1.23 & 0 & 4.72 & \textbf{8.42} & 1.64 & 0.41 & 3.08 & 3.29 & 1.03 & 0 \\
        ORLM, PoT+CoT, Implicit(\%) & 1.21 & 0.60 & 0 & 2.42 & 5.04 & 2.22 & 0 & \textbf{7.66} & 1.81 & 0.40 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 1.21 & 1.21 & 0 & 3.74 & 4.47 & 2.66 & 0.24 & \textbf{10.02} & 1.33 & 0.60 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 1.19 & 2.27 & 0 & 3.22 & 3.34 & 2.27 & 0.36 & \textbf{5.85} & 1.79 & 0.48 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 31.47 & 0 & 0 & 2.10 & \textbf{34.97} & 0 & 1.40 & 4.90 & 25.17 & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & 17.88 & 1.12 & 0 & 4.47 & 12.85 & 0 & 0 & 0 & \textbf{18.44} & 0 & 0 \\
        \bottomrule
    \end{tabular}}
    \label{tab24}
\end{table}

\begin{table}[ht]
    \centering
    \caption{2D-cutting packing-constrained guillotine Problems Performance Metrics}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lccccccccccc@{}}
        \toprule
        \textbf{Models, Techniques and Expression} & \textbf{IndexError(\%)} & \textbf{FileNotFoundError(\%)} & \textbf{OverflowError(\%)} & \textbf{NameError(\%)} & \textbf{ValueError(\%)} & \textbf{AttributeError(\%)}& \textbf{KeyError(\%)}& \textbf{SyntaxError(\%)}& \textbf{TypeError(\%)}& \textbf{ImportError(\%)}& \textbf{PulpError(\%)} \\ 
        \midrule
        \rowcolor{gray!20}
        GPT-4o-mini, PoT+CoT, Explicit & 0 & 0 & 0 & 0 & \textbf{57.14} & 0 & 0 & 0 & 42.86 & 0 & 0 \\ 
        \hdashline
        GPT-4o-mini, PoT, Implicit & 16.67 & 0 & 0 & 0 & \textbf{33.33} & 0 & 0 & 16.67 & \textbf{33.33} & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit & 10 & 0 & 0 & 10 & \textbf{70} & 2.37 & 0 & 0 & 0 & 0 & 0 \\
        GPT-4o-mini, PoT+CoT, Implicit-disorder & 3.23 & 0 & 0 & 0 & \textbf{19.35} & 0 & 0 & 0 & 0 & 0 & 0 \\
        LLAMA3-8B, PoT, Implicit & 2.51 & 0 & 0 & 1.76 & 7.40 & 5.27 & 6.52 & \textbf{17.69} & 4.77 & 0.50 & 0 \\ 
        LLAMA3-8B, PoT+CoT, Implicit(\%) & 0 & 0 & 0 & 4.35 & 8.70 & 13.04 & 0 & 0 & \textbf{17.39} & 0 & 0 \\
        LLAMA3-8B, PoT, Implicit-disorder(\%) & 6.90 & 0 & 0 & 6.90 & \textbf{58.62}& 6.90 &3.45 & 0 & 13.79 & 0 & 0 \\
        LLAMA3-8B, PoT+CoT, Implicit-disorder(\%) & 0 & 0 &\textbf{ \textbf{0}} & 6.06 & \textbf{39.39} & 6.06 & 0 & 6.06 & 36.36 & 0 & 0 \\
        ORLM, PoT, Implicit(\%) & 0 & 1.18 & 0 & 1.18 & 0 & 0 & 1.18 & 1.18 & 2.35 & 0 & 0 \\
        ORLM, PoT+CoT, Implicit(\%) & 0 & 1.18 & 0 & 1.18  & \textbf{3.53} & 0 & 0 & 4.71 & 1.18 & 0 & 0 \\
        ORLM, PoT, Implicit-disorder(\%) & 0 & 0.70 & 0 & 0.70 & 4.90 & 3.50 & 0.70 & \textbf{6.29} & 2.10 & 0 & 0 \\
        ORLM, PoT+CoT, Implicit-disorder(\%) & 6.90 & 0 & 0 & 6.90 & \textbf{58.62} & 6.90 & 3.45 & 0 & 13.79 & 0 & 0 \\
        DeepSeek-R1, PoT, Implicit(\%) & 15.91 & 0 & 0 & 0 & 22.73 & 0 & 0 & 2.27 & \textbf{40.91} & 0 & 0 \\
        DeepSeek-R1, PoT+CoT, Implicit(\%) & 3.32 & 1.85 & 0 & 3.32 & 8.86 & 4.06 & 0.37 & \textbf{9.59} & 4.06 & 0.74 & 0 \\
        \bottomrule
    \end{tabular}}
    \label{tab26}
\end{table}








